Recursive Bayesian Filters for Data Assimilation

A thesis on some recursive Bayesian filters for data assimilation

==> abst.tex <==

\chapter*{\centering Abstract}
\thispagestyle{empty} 
%\begin{abstract}
Data assimilation refers to any approach designed to improve the estimation of system states or parameters by exploiting the additional information contained in the observations of a dynamical system. In practice, a mathematical model is often not the precise description of the underlying physical process for various reasons. In this case, data assimilation can be used to narrow the gap between estimations from a mathematical model and reality.

In data assimilation applications, one is often confronted by three problems: nonlinearity, non-Gaussianity and high dimensionality (for example, a weather forecasting model may have over millions of state variables). This dissertation is thus dedicated to studying some data assimilation methods that aim to address these problems.

First of all we consider two types of nonlinear Kalman filters, the ensemble Kalman filter (EnKF) and the sigma point Kalman filter (SPKF), for data assimilation in nonlinear Gaussian systems. To reduced the computational cost of the SPKF in high dimensional systems, we introduce the reduced rank version of the SPKF.  

Then we proceed to study the Gaussian sum filter (GSF) for data assimilation in nonlinear non-Gaussian systems. It can be shown that a GSF essentially consists of a set of parallel nonlinear Kalman filters. For this reason, we call a type of nonlinear Kalman filter a ``base filter'' of the GSF. The aforementioned EnKF and reduced rank SPKF can both be used as base filters of a GSF. To reduce the potential computational cost and increase the numerical stability of a GSF, we also propose an auxiliary algorithm. We show that, if the reduced rank SPKF-based GSF is equipped with the auxiliary algorithm and implemented in parallel, it can achieve almost the same computational speed as that of the reduced rank SPKF itself. With suitable parameters in the reduced rank SPKF-based GSF or the EnKF-based GSF, the GSF normally outperforms its base filter.    
%\end{abstract}   

==> ackno.tex <==

\chapter*{\centering Acknowledgements}
\thispagestyle{empty} 
%\begin{acknowledgements}
First, I would like to thank my parents for their endless support and love. I am also deeply grateful to my wife Xiaoping for her patience and support. Without them I could not have completed this research.

I thank my supervisor, Dr Irene Moroz, for her guidance and encouragement in my research, and for her efforts in advocating me to attend various seminars, workshops and conferences. The interactions with so many kind and encouraging researchers always benefited my own study. Special thanks to Dr Chris Farmer, who urged me to investigate the Gaussian sum filtering methods in this research. I also thank Dr John Norbury, who gave me a wonderful experience in undergraduate teaching and has continued to be supportive for my research over the last three years.

Finally, I would like to thank all my friends in Oxford, with special thanks to Judy, Laura, Lian, Mohammed, Oscar, Reason, Shuli, and Trevor in ADS\&IP group of OCIAM for their enduring friendship.
%\end{acknowledgements}



  
